Knowledge Probing for Graph Representation Learning

Graph learning methods have been extensively applied in diverse application areas. However, what kind of inherent graph properties e.g. graph proximity, graph structural information has been encoded into graph representation learning for downstream tasks is still under-explored. In this paper, we propose a novel graph probing framework (GraphProbe) to investigate and interpret whether the family of graph learning methods has encoded different levels of knowledge in graph representation learning. Based on the intrinsic properties of graphs, we design three probes to systematically investigate the graph representation learning process from different perspectives, respectively the node-wise level, the path-wise level, and the structural level. We construct a thorough evaluation benchmark with nine representative graph learning methods from random walk based approaches, basic graph neural networks and self-supervised graph methods, and probe them on six benchmark datasets for node classification, link prediction and graph classification. The experimental evaluation verify that GraphProbe can estimate the capability of graph representation learning. Remaking results have been concluded: GCN and WeightedGCN methods are relatively versatile methods achieving better results with respect to different tasks.

==> 2_background.tex <==
% \pdfoutput=1
\section{Background}

% \subsection{Graph Embedding Model}
% Graph embedding is a technique that maps graph data (usually high-dimensional dense matrices) to low-dimensional dense vectors, which can solve the problem of graph data being difficult to efficiently input into machine learning algorithms. Graph embedding can capture the topology structure, vertex-to-vertex relationships and other relevant information about the graph, subgraph and vertices.

% \subsection{Weisfeiler-Lehman isomorphism test}
% The Weisfeiler-Lehman (WL) isomorphism test is a graph isomorphism test based on color refinement. It iteratively assigns colors (or labels) to the nodes of two graphs, based on their initial colors and the colors of their neighbors. If the color distributions of the two graphs are different at any iteration, then they are not isomorphic.

% The WL test can also be used to define graph kernels, which are similarity measures between graphs that can be used for graph classification or regression tasks. The general WL kernel framework consists of three steps: (1) relabeling the nodes of each graph using the WL test, (2) computing a feature vector for each graph based on the node labels, and (3) computing a kernel value between two graphs based on their feature vectors.

% \subsection{Supervised Contrastive Learning}
% Supervised Contrastive Learning (SCL) is a training methodology that extends the self-supervised batch contrastive approach to the fully-supervised setting, allowing to effectively leverage label information for representation learning. SCL uses a supervised contrastive (SupCon) loss, which pulls together clusters of points belonging to the same class in embedding space, while simultaneously pushing apart clusters of samples from different classes.
